Tailoring with Targeted Precision: Edit-Based Agents for Open-Domain Procedure Customization

How-to procedures, such as how to plant a garden, are now used by millions of users, but sometimes need customizing to meet a user's specific needs, e.g., planting a garden without pesticides. Our goal is to measure and improve an LLM's ability to perform such customization. Our approach is to test several simple multi-LLM-agent architectures for customization, as well as an end-to-end LLM, using a new evaluation set, called CustomPlans, of over 200 WikiHow procedures each with a customization need. We find that a simple architecture with two LLM agents used sequentially performs best, one that edits a generic how-to procedure and one that verifies its executability, significantly outperforming (10.5% absolute) an end-to-end prompted LLM. This suggests that LLMs can be configured reasonably effectively for procedure customization. This also suggests that multi-agent editing architectures may be worth exploring further for other customization applications (e.g. coding, creative writing) in the future.

==> tables/qual_analysis.tex <==
\begin{table*}
    \centering
    \begin{tabular}{|c|r|r|r|}
    \hline
         & \cust & \exec & \fc \\ \hline
         % E2E generate-customize&  52.5\%&  75\%& 40\%\\
         E2E customize&  60\%&  72.5\%& 47.5\%\\ \hline
         % Customized edits only&  55\%&  85\%& 50\%\\
         \uniagent &  52.5\%&  90\%& 47.5\%\\
         \seqagents &  62.5\%&  90\%& 55\%\\
         Reverse \seqagents &  52.5\%&  87.5\%& 40\%\\
         \paragents &  62.5\%&  70\%& 50\%\\ \hline
    \end{tabular}
    \caption{Qualitative judgments of different methods on data sample in \S\ref{sec:e2e-llms-eval}. 
    Trends across methods on this data sample match the trends on the full dataset, reinforcing our method of performing qualitative analysis.
    }
    \label{tab:qual_eval}
\end{table*}

==> tables/qual_e2e.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{|c|r|r|r|}
    \hline
         &  \fc \\ \hline
         E2E generate-customize& 40\%\\
         E2E customize& 47.5\%\\ \hline
    \end{tabular}
    \caption{Qualitative analysis of plans generated by end-to-end approaches to customization using \llm s \niket{do not need a table.}}
    \label{tab:qual_eval_e2e}
\end{table}
